Predicting generalization performance with correctness discriminators

The ability to predict an NLP model's accuracy on unseen, potentially out-of-distribution data is a prerequisite for trustworthiness. We present a novel model that establishes upper and lower bounds on the accuracy, without requiring gold labels for the unseen data. We achieve this by training a discriminator which predicts whether the output of a given sequence-to-sequence model is correct or not. We show across a variety of tagging, parsing, and semantic parsing tasks that the gold accuracy is reliably between the predicted upper and lower bounds, and that these bounds are remarkably close together.

==> resubmission_response.tex <==
According to the area chair, our paper investigates an important research question, provides a sound methodology and shows good results.
The main suggestions from the area chair is to (1) have a discussion of the epistemic problem of using a trained model to judge the accuracy of a trained model and (2) address the unnecessary overhead to use seq2seq to solve the classification task.
Hence, we make following changes to address them.
\begin{itemize}
    \item We include new results where we use a RoBERTa-based discriminator to predict performance across our datasets.
    \item We add a discussion of the legitimacy of using a trained model to judge the accuracy of a trained model.
    \item We revise the description of our ensemble method to clarify its mechanism clearly.  
\end{itemize}

==> sections/Dataset_details_and_baseline.tex <==
\section{Dataset Details and Baseline}

We mainly experiment with three datasets: GeoQuery, COGS, CFQ, TOP and AMR2.0. Examples for each dataset are present in Table \ref{fig:data_example}. For each dataset, we run a T5-base model as baseline parser and report its exact match accuracy in Table \ref{tab:baseline_results}. 

\paragraph{Details for AMR parsing.} For AMR, the common evaluation metric is Smatch \cite{cai-knight-2013-smatch}. We adopt the same preprocessing setting like \cite{graphene}. Our parser achieves 78.1\% (T5-base) and 80.7\% (T5-large) Smatch F score, compared to the 83.0\% in \cite{graphene} (T5-large). Although our parser does not achieve very strong performance, it should not be bad as a baseline for experiments in this report.

% \input{tables/baseline_results}
\input{tables/dataset_examples}


==> sections/Discrim_test_set.tex <==
% \subsection{Use discriminator for data augmentation}
% Our backtranslation-based data augmentation yields a lot of noisy data since the input is generated by backtranslation. Assuming we have a good discriminator, can we use it to filter those incorrect instances out from augmented data? To answer this question, we also experiment this idea on GeoQuery. Current results show no difference between filtered and unfiltered settings, with both models achieving 84\% accuracy on test set. One possible reason is that our discriminator performs bad on GeoQuery, and thus even the filtered data still contains much noise. Also, the backtranslation model may not be able to output correct instances for most sentences.  

\section{Use discriminator to predict model accuracy on test set}
\subsection{Increase Incorrect-Recall score} \label{sec:discrim_test:ir}
\input{tables/discrim/hyperparam_explore}

Our discriminator can also be used to predict the accuracy of our semantic parser on test set, where an instance is counted as \textit{correct} if the discriminator predict it as \textit{correct}. 
So far we have seen that our discriminator can achieve almost 100\% \textit{Correct-Recall} on MCD1 and COGS. Based on this, we can calculate the upperbound accuracy of our semantic parser on test set. Can we instead get a discriminator with \textit{Incorrect-Recall} close to 100\%, so that the discriminator can discover all truly incorrect instances to calculate the lowerbound accuracy on test set?

We consider three settings here with T5: training data, the ratio of negative to positive samples, and ensemble. For training data, since \textit{Model} method seems more promising in Table \ref{tab:discrim_results}, we focus on this method in this experiment. Here we consider model checkpoints trained after fixed steps used to generate training data. Thus, a model checkpoint at 2k steps is denoted as $M_{2k}$.  For the ratio setting, we experiment with larger ratio of negative to positive samples (i.e.\ 3:1). For ensemble, we train multiple models with different random seeds (i.e.\ 0-4) and combine their predictions for the same instance. Generally such combination is implemented with a \textit{vote} mechanism. Since our purpose here is to yield higher \textit{Incorrect-recall}, we instead combine predictions such that an instance is labeled as \textit{Incorrect} if there exists a model prediction being \textit{Incorrect}. We call this combination mechanism \textit{vote\_incorrect}. Similarly, we can combine predictions such that an instance is labeled as \textit{Correct} if there exists a model prediction being \textit{Correct}, which we call \textit{vote\_correct}.  

% We also experiment with a classification model, where the encoder is a transformer with roberta-base representations.
Table \ref{tab:discrim:hyperparam_explore} shows results for these settings. First we can observe that both increasing ratio of negative examples and ensemble can benefit \textit{Incorrect-recall} scores and combining both methods yields the best score on all datasets. On CFQ splits, using checkpoint $M_{2k}$ gives a good enough result. On COGS, checkpoints selection gives a large impact on the resulted IR score (i.e.\ 78 with $M_{25k}$ v.s.\ 94 with $M_{0.5k}$).

The observation that $M_{0.5k}$ outperforms $M_{2k}$ raises a question: is it generally better to collect errors in the early training stage than the end of training? To investigate this question, we present results of models trained on data generated according to different checkpoints in Table \ref{tab:discrim:ckpt}. Here we do not use ensemble and adopt ratio of negative examples 3:1. We can observe that compared to the checkpoint at the end of training, early-stage checkpoints lead to better performance and combining them gives the best IR score (i.e. 97) on COGS.

\subsection{Predict test-set accuracy}

Given the findings so far, we can now predict the upperbound and lowerbound of accuracy of our parser on test set. Our settings are introduced below.

\paragraph{Models}
We use the same discriminator as our predictor for both upperbound and lowerbound. Following the finding in section \ref{sec:discrim_test:ir}, we train T5-base with training data generated by \textit{Comb} method, ratio of negative examples being 3:1 and number of ensemble models being 5. \textit{vote\_incorrect} is used to predict the lowerbound and \textit{vote\_correct} is used to predict the upperbound.

\paragraph{Datasets}
We mainly focused on compositional generalization tasks so far. Is is possible to extend our idea to other datasets or tasks? Which scenarios should we expect our method work? Here we consider several conditions that the task should meet: 
1) The output of the task should be a sequence. This is because we expect the model to learn to discriminate between input sequence to output sequence. For a classification task, the output label should not give much information. 
2) The correctness of the task output sequence should be defined clearly. For tasks such as machine translation or text summarization, it is hard to define the correctness of an output sequence, which will introduce additional difficulty for training the discriminator.
3) Discriminating an output sequence should be challenging enough. For tasks like controlled text generation, discriminating can be easily implemented with a simple heuristic (i.e.\ calculate output sequence length), and thus we do not need a discriminator to do this.

\input{tables/discrim/test_acc}

\input{tables/discrim/ckpt}

Given reasons above, we mainly focus on semantic parsing tasks, and extend our datasets with two more tasks: TOPv2 \cite{chen-etal-2020-low} and AMR 2.0 \cite{banarescu-etal-2013-abstract}. TOPv2 is a low-resource domain adaptation task and we use its \textit{weather} split with 176 training sentences and 147 test sentences. AMR 2.0 is a broad-coverage semantic parsing task and we use its official split with 36521 training sentences and 1371 test sentences.   

\paragraph{Related method} Previous works also use maximal output probability of the seq2seq parser as model confidence about whether the prediction is correct or not. A discriminator can be implemented by setting a threshold $\gamma$ and make predictions by comparing $\gamma$ and the confidence score. Such method is defined as \textit{Maxprob} in \cite{kamath-etal-2020-selective}. Here we also report the result of \textit{Maxprob} with $\gamma=0.5$. \todo{I did not list here but there are other possible methods to do discriminator such as calibration methods.}


\paragraph{Results}
Table \ref{tab:discrim:test_acc} reports the predicted accuracy.

\input{tables/discrim/conf_interval}
\paragraph{Confidence Interval}
% Our discriminator is not perfect since it cannot achieve 100\% CR or IR scores.
Is it possible to evaluate the confidence interval of our discriminator? The most common way to calculate this is \textit{bootstrapping}. Here we do this by sampling 1000 predictions of the entire test set based on the predicted probability by the discriminator, calculating their accuracy, ranking accuracy list and then selecting 25th and 975th predicted accuracy as the lowerbound and upperbound of a 95\% confidence interval. We report some results in Table \ref{tab:discrim:conf}. Here we do not use ensemble since it is not clear yet how to do bootstrapping for ensemble models.

\paragraph{Error analysis}
I also did some error analysis on the misclassified instances by the discriminator. Some examples on TOP and AMR are shown in Table \ref{fig:discrim:error}. Currently I only present errors made by the lowerbound discriminator. This means that the discriminator gives a high Incorrect-Recall and high Correct-Precision. Here I present the truly incorrect instances that is predicted as correct for our discriminator.

\input{tables/discrim/error_analysis}
\subsection{Next step}

\input{figures/acc_vs_scale/fig}

% \todo{1. Add Syntactic parsing and POS tagging with Penntreebank dataset}

% \todo{2. Compare with more thresholds or other previous methods}

% \todo{3. }

\paragraph{Improving the IR/CR scores and comparing with previous methods}. In addition to \textit{Maxprob}, there are other possible ways to construct discriminator in calibration works and perhaps other areas. I think it will make our point more strong if we can compare with more methods. Also, there is still space to improve our current discriminator so we can spend more time on that.

\paragraph{Investigate why our method works}. It will also be interesting to answer why our method works well. Do our collected training errors already cover most possible errors the parser made on the test set so the generalization gap is small? If so, can we think of a more clever way to collect training errors as the training set? One possibly related observation is that when a parser gets 0 loss on the train set, most errors we can collect on the train set are out-of-vocabulary errors (i.e. replacing a correct word with similar words) rather than structure errors, which may not be what we want. We have also discussed investigating the distance between error distributions on train and test set, which could also be related. 

\paragraph{Try more models}. In some pilot study I found that T5-large generally outperforms T5-base not only as a semantic parser but also for discriminator. I think it will also be interesting to see the effect of LLM. A lora-finetuned llama should already be enough. Not sure if we want to try GPT-4 and in-context learning.

\paragraph{Downstream applications}. Our method can naturally be used for different purposes. Here are some I can think now: 
1) Validation for compositional generalization is hard because for some tasks no annotated test-distribution data are available. To address this, we can assume that we have access to at least some test-distribution input sentences and thus we can validate on the model predictions on such sentences with our discriminator. 
2) Continual training. Assuming we have a high Correct-Precision discriminator and unlimited input sentences from test-set distribution, we can easily get model predictions on these sentences and only maintain correct ones with our discriminator. These high-quality annotated data can be further included in the train set of our parser to improve performance.
3) Finding valuable instances for annotation. Assuming we have a high Incorrect-Precision discriminator and unlimited input sentences from test-set distribution, we can easily find sentences which tends to be incorrectly predicted. Such instances can be further annotated by humans to effectively improve model performance.  

==> sections/Discriminator.tex <==
\section{Discriminator}
Task definition: Mapping a pair of natural language sentence and a meaning representation into a binary class (e.g. X -> {\textit{Correct}, \textit{Incorrect}}).

\subsection{Training discriminator with synthetic data}  \label{sec:discrim:train}

\paragraph{Synthesized training data.}
Create train sets for both GeoQuery and MCD1 with two versions to generate negative samples in training: \textit{Random} and \textit{Model}.

1. \textit{Random} means for an example in Table \ref{fig:data_example}, we insert (random conjunct) and delete each conjunct with a probability=0.2. We apply this on the original train set and test set of MCD1 splilt and use the resulted dataset as the new train and test sets. The proportion of negative examples in the resulted datasets is 50\%.

2. \textit{Model} means for an example below, we first train an T5 parser on the train set of original MCD1 train set, and then take the incorrect predicted meaning representations maintained in the beam of decoder with the highest probability as the negative example. We apply this on the original train set and test set of MCD1 splilt and use the resulted dataset as the new train and test sets. The proportion of negative examples in the resulted datasets is 50\%.

\paragraph{Test data}
We use the the output from the baseline T5 parser to construct test set. Specifically, the test set of this discriminator task shares the same size as the test set of semantic parsing task. The input is the concatenation of English sentence and predicted meaning representation from the baseline parser. The output is a Correct/Incorrect label indicating whether the prediction is correct or not.  

\paragraph{Metrics} 
% For all parser tasks, we evaluate the exact match accuracy of our parser. For the discriminator, we evaluate its predicted accuracy on the test, which should be the exact match accuracy by the corresponding parser.
\todo{Do we need a MAE }
We evaluate \textit{Precision} and \textit{Recall} for the discriminator individually. For \textit{Precision} and \textit{Recall}, we report the score for \textit{Correct} and \textit{Incorrect} label individually. 
We define \textit{Truely Correct (TC)} as instances with annotation being \textit{Correct} and the prediction being \textit{Correct}, \textit{Falsely Correct (FC)} as instances with annotation being \textit{incorrect} and the prediction being \textit{correct}. Thus the \textit{Correct-Precision} is calculated as below. The scores for \textit{Incorrect} label is calculated with the same way.
\begin{equation}
    Count(TC)/(Count(TC)+Count(FC))
\end{equation}

\paragraph{Results} Results are reported in Table \ref{tab:discrim_results}. We can observe that the T5 discriminator works well on MCD1 and COGS. According to the \textit{Incorrect-Recall} score, 76\% incorrect predictions on MCD1 can be recognized by the discriminator and 72\% for COGS.

\input{tables/discrim_results}


==> sections/Refine.tex <==
\section{Refine}
Task definition: Mapping a pair of natural language sentence and an incorrect meaning representation into a meaning representation (e.g. X, Y -> Y*).

\subsection{Training refine model with synthetic data}
\paragraph{Synthesized training data.}
Here we follow similar methods as described in Section \ref{sec:discrim:train}.

\paragraph{Test data}
We use the incorrect predictions from the baseline T5 parser to construct our test set. The input is the concatenation of an input sentence from the original test set and the output is the incorrect prediction from T5 parser. 

\paragraph{Metrics}
We use exact match accuracy as evaluation metrics.

\paragraph{Results}
We report results in Table \ref{tab:refine_results}. Currently the refine model does not work well.

\input{tables/refine_results}



==> tables/baseline_results.tex <==
\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{lXXXXX}
    \toprule
     & COGS & CFQ & GeoQuery & TOP & AMR2.0\\
     \cmidrule[0.5pt](l){2-6}
     % \cmidrule{}
     & Gen & MCD1 & Template & Weather & Test \\
    \midrule
    T5 & 92 & 58 & 80 & 73 & 12 \\ 
    \bottomrule
    \end{tabularx}
    \caption{Exact match accuracy of baseline models.
    % \todo{plan to add results with additional MRs from dev set.} 
    % \todo{update numbers}
    }
    \label{tab:baseline_results}
\end{table}

==> tables/dataset_examples.tex <==
\begin{table*}
    \centering
    \footnotesize
    \begin{tabular}{@{}llm{.7\linewidth}@{}}
        \toprule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{Geo}} &  {Input} & {what state has the largest population density ?}  \\
         \cmidrule(l){2-3}
          &  {Output} &  {\lform{answer ( largest\_one ( density\_1 ( state ( all ) ) ) )}} \\
         \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{CFQ}} &  {Input} & {Did M0 ' s writer write M1 and M2}  \\
         \cmidrule(l){2-3}
          &  {Output} &  {\lform{SELECT count ( * ) WHERE lb ?x0 film.writer.film M0 . ?x0 film.writer.film M1 . ?x0 film.writer.film M2 rb}} \\
          \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{COGS}} &  {Input} & {The baby on a tray in the house screamed.}  \\
         \cmidrule(l){2-3}
          &  {Output} &  {\lform{ scream ( agent = * baby ( nmod . on = tray ( nmod . in = * house ) ) )}} \\
          \midrule
          \multirow{2}{*}{\rotatebox[origin=c]{90}{TOP}} &  {Input} & {Will there be snowfall this week?}  \\
         \cmidrule(l){2-3}
          &  {Output} &  {\lform{[in:get\_weather will there be [ sl:weather\_attribute snowfall ] [ sl:date\_time this week ] ? ]}} \\
          \midrule
          \multirow{2}{*}{\rotatebox[origin=c]{90}{AMR}} &  {Input} & {Did Palin apologize to Giffords?}  \\
         \cmidrule(l){2-3}
          &  {Output} &  {\lform{( apologize-01 :mode interrogative :ARG0 ( person\_0 :name ( name\_0 :op1 "Palin" ) ) :ARG2 ( person\_1 :name ( name\_1 :op1 "Giffords" ) ) )}} \\
         \bottomrule
    \end{tabular} 
    \caption{ }
    \label{fig:data_example}
\end{table*}

==> tables/discrim/ckpt.tex <==
\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{XXXXXXX}
    \toprule
         &\multicolumn{2}{c}{COGS} & \multicolumn{2}{c}{MCD1} & \multicolumn{2}{c}{MCD2} \\
         \cmidrule(lr){2-3}
         \cmidrule(lr){4-5}
         \cmidrule(lr){6-7}
     Ckpt & CR & IR  & CR & IR  & CR & IR \\
     \midrule
     M_{e1} & 100 & 6 & 98 & 74& 79& 80 \\
     M_{e2} & 100 & 53& 98& 82& 77& 83\\
     M_{e3} & 100 & 90& 98& 75& 79& 83\\
     M_{e4} & 100 & 91& 97& 79& 76& 83\\
     M_{e5} & 100 & 87& 98& 83& 81& 81\\
     Comb & 99& \textbf{97} & 97& \textbf{83} & 81 & \textbf{84} \\
     M_{end} & 100 & 72 & - & - & - & - \\
    \bottomrule
    \end{tabularx}
    \caption{\textit{Correct-Recall} and \textit{Incorrect-Recall} scores with regard to training data generated from different checkpoints. The score is calculated with a single model instead of ensemble. $M_{e1}$ refers to the checkpoint after the first training epoch and so for others. \textit{Comb} means we combine all training data generated by $M_{e1}$-$M_{e5}$. $M_{end}$ refers to the checkpoint at the end of training. \todo{Todo: get numbers on CFQ}}
    \label{tab:discrim:ckpt}
\end{table}



==> tables/discrim/conf_interval.tex <==
\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{XXXX}
    \toprule
         &\multicolumn{1}{c}{COGS} & \multicolumn{1}{c}{MCD1} & \multicolumn{1}{c}{MCD2} \\
         % \cmidrule(lr){2-3}
         % \cmidrule(lr){4-5}
         % \cmidrule(lr){6-7}
      & \multicolumn{3}{c}{Predicted Acc} \\
     \midrule
     Discriminator & 90.3 & 63.1 & 31.0  \\
     Upper. \tiny(Conf 95\%) & 90.4 & 63.3 & 31.2 \\
     Lower. \tiny(Conf 95\%) & 90.3 & 62.9 & 30.8 \\
    \bottomrule
    \end{tabularx}
    \caption{}
    \label{tab:discrim:conf}
\end{table}

==> tables/discrim/error_analysis.tex <==
\begin{table*}
    \centering
    \footnotesize
    \begin{tabular}{@{}llm{.7\linewidth}@{}}
        \toprule
          \multirow{5}{*}{\rotatebox[origin=c]{90}{TOP}} &  {Input} & {What degrees Fahrenheit is it outside?}  \\
         \cmidrule(l){2-3}
          &  {Parser} &  {\lform{[ in:get\_weather what degrees [ sl:weather\_temperature\_unit fahrenheit ] is it outside ? ]}} \\
          \cmidrule(l){2-3}
          & {Discrim (high CP)} & {Correct} \\
          \cmidrule(l){2-3}
          &  {Anno} &  {\lform{[ in:get\_weather what [ sl:weather\_temperature\_unit degrees fahrenheit ] is it outside ? ]}} \\
          \cmidrule(l){2-3}
          & {Gold} & {Incorrect} \\
          \midrule
          \multirow{5}{*}{\rotatebox[origin=c]{90}{AMR}} &  {Input} & {2003-06-24}  \\
          \cmidrule(l){2-3}
          & {Parser} & {\lform{( date-entity :year 2003 :month 6 :day 24 )}} \\
          \cmidrule(l){2-3}
          & {Discrim (high CP)} & {Correct} \\
          \cmidrule(l){2-3}
          & {Anno} & \lform{( date-entity :month 6 :day 24 :year 2003 )} \\
          \cmidrule(l){2-3}
          & {Gold} & {Incorrect} \\
          \midrule
            \multirow{5}{*}{\rotatebox[origin=c]{90}{AMR}} &  {Input} & {Thanks for reading.}  \\
          \cmidrule(l){2-3}
          & {Parser} & {\lform{( thank-01 :ARG0 ( i ) :ARG1 ( you ) :ARG2 ( read-01 :ARG0 you ) )}} \\
          \cmidrule(l){2-3}
          & {Discrim (high CP)} & {Correct} \\
          \cmidrule(l){2-3}
          & {Anno} & \lform{( thank-01 :ARG1 ( you ) :ARG2 ( read-01 :ARG0 you ) )} \\
          \cmidrule(l){2-3}
          & {Gold} & {Incorrect} \\
         
         \bottomrule
    \end{tabular} 
    \caption{Error analysis}
    \label{fig:discrim:error}
\end{table*}

==> tables/discrim/hyperparam_explore.tex <==



==> tables/discrim/test_acc.tex <==
% \begin{table*}
% \footnotesize
%     \centering
%     \begin{tabularx}{\linewidth}{XXXXXXXXXXXXXXXX}
%     \toprule
%      & \multicolumn{3}{c}{MCD1} & \multicolumn{3}{c}{MCD2} & \multicolumn{3}{c}{COGS} & \multicolumn{3}{c}{Top} & \multicolumn{3}{c}{AMR2.0}\\
%      \cmidrule(lr){2-4}
%      \cmidrule(lr){5-7}
%      \cmidrule(lr){8-10}
%      \cmidrule(lr){11-13}
%      \cmidrule(lr){14-16}
%      & CR & IR  & Acc & CR & IR & Acc & CR & IR & Acc & CR & IR & Acc & CR & IR & Acc\\
%     \midrule
%     \multicolumn{16}{l}{\textit{Maxprob}} \\
%     $\gamma$=0.25 & 99.9 & 10.4 & 95.5 & \textbf{99.9} & 7.7 & 94.0  & 100 & 6.0 & 99.5 & 100 & 2.6 & 99.3 & \textbf{99.4} & 43.3 & 61.9 \\
%     $\gamma$=0.50 & 98.7 & 35.0 & 84.5 & 96.7 & 27.6 & 78.0  & 99.8 & 32.0 & 97.1 & 98.1 & 23.7 & 92.2 & 96.4 & 67.2 & 40.6 \\
%     $\gamma$=0.75 & 94.8 & 59.9 & 71.7 & 87.1 & 51.9 & 57.0  & 99.2 & 57.2 & 94.4 & 85.4 & 63.2 & 72.3 & 87.3 & 82.5 & 26.1 \\
%     \midrule
%     \multicolumn{16}{l}{\textit{Maxprob (Oracle)}} \\
%     Upper. &99.2 & 31.2 & 86.4 &  83.4 & 58.3 & 51.3  & 99.8 & 36.6 & 96.7 & 92.2 & 31.6 & 85.8 & 71.0 & 90.9 & 17.9 \\
%     Lower. & 75.5 & 92.9 & 46.6 &  48.7 & 92.2 & 17.2 & 48.2 & 96.9 & 44.3 & 81.6 & 78.9 & 65.2 & 35.2 & 99.1 & 5.8 \\
%     \midrule
%     \multicolumn{16}{l}{Ours} \\
%     Upper. & \textbf{99.2} & 69.8 & 70.0 & 83.4 & 77.9 & 36.1 & \textbf{99.8} & 89.4 & 92.1 & \textbf{92.2} & 44.7 & 82.3 & 70.9 & 84.1 & 22.6 \\
%     Lower. & 92.9 & \textbf{94.5} & 56.0 & 71.7 & \textbf{92.2} & 22.4 & 98.5 & \textbf{96.9} & 90.2 & 82.5 & \textbf{78.9} & 66.0 & 29.1 & \textbf{99.1} & 4.5 \\
%     \midrule
%     Gold & - & - & 57.8 & - & - & 22.9  & -& - & 91.4 & - & -& 73.0 & - & - & 12.2 \\

%     \bottomrule
%     \end{tabularx}
%     \caption{Predicted test-set accuracy with different methods. \textit{Maxp} refers to using the maximum predicted probability as discriminator. \textit{Upper.} and \textit{Lower.} refers to predicted upperbound and lowerbound. \textit{Gold} refers to the accuracy evaluated with gold annotations. }
%     \label{tab:discrim:test_acc}
% \end{table*}


% \begin{table*}
% \footnotesize
%     \centering
%     \begin{tabularx}{\linewidth}{XXXXXXXXXX}
%     \toprule
%      &  & \multicolumn{3}{c}{\textit{Maxprob}} & \multicolumn{2}{c}{\textit{Maxprob (Oracle)}} & \multicolumn{2}{c}{Ours} & Gold \\
%      \cmidrule(lr){3-5}
%      \cmidrule(lr){6-7}
%      \cmidrule(lr){8-9}
%     Data & Metric & $\gamma$=0.25 & $\gamma$=0.5 & $\gamma$=0.75 & Upper. & Lower. & Upper. & Lower. & \\ 
%     \midrule
%     \multirow{3}{}{MCD1} & CR  & 99.9 & 98.7 & 94.8 & 99.2 & 71.7 & 99.2 & 92.9 & - \\
%     & IR & 10.4 & 35.0 & 59.9 & 31.2 & 94.5 & 69.8 & 94.5 & - \\
%     & Acc & 95.5 & 84.5 & 71.7 & 86.4 & 43.7 & 70.0 & 56.0 & 57.8 \\
%     \midrule
%     \multirow{3}{}{MCD2} & CR  & 99.9 & 96.7 & 87.1 & 83.4 & 48.7 & 83.4 & 71.7 & -  \\
%     & IR & 7.7 & 27.6 & 51.9 & 58.3 & 92.2 & 77.9 & 92.2 & - \\
%     & Acc & 94.0 & 78.0& 57.0 & 51.3 & 17.2 & 36.1 & 22.4 & 22.9 \\
%     \midrule
%     \multirow{3}{}{COGS} & CR  & 100 & 99.8 & 99.2 & 99.8 & 48.2 & 99.8 & 98.5 & - \\
%     & IR & 6.0 & 32.0 & 57.2 & 36.6 & 96.9 & 89.4 & 96.9 & - \\
%     & Acc & 99.5 & 97.1 & 94.4 & 96.7 & 44.3 & 92.1 & 90.2 & 91.4 \\
%     \midrule
%     \multirow{3}{}{Top} & CR  & 100 & 98.1 & 85.4 & 92.2 & 81.6 & 92.2 & 82.5 & - \\
%     & IR & 2.6 & 23.7 & 63.2 & 31.6 & 78.9 & 44.7 & 78.9 & - \\
%     & Acc & 99.3 & 92.2 & 72.3 & 85.8 & 65.2 & 82.3 & 66.0 & 73.0 \\
%     \midrule
%     \multirow{3}{}{AMR} & CR  & 99.4 & 96.4 & 87.3 & 71.0 & 35.2 & 70.9 & 29.1 & - \\
%     & IR & 43.3 & 67.2 & 82.5 & 90.9 & 99.1 & 84.1 & 99.1 & - \\
%     & Acc & 61.9 & 40.6 & 26.1 & 17.9 & 5.8 & 22.6 & 4.5 & 12.2 \\
%     \midrule
%     \multirow{3}{}{POS-WSJ} & CR & 99.9 & 94.4 & 77.9 & 93.0 & 65.3 & 93.0 & 52.4 & - \\
%     & IR & 3.9 & 33.3 & 72.4 & 37.5 & 84.8 &  26.5 & 84.8 & - \\
%     & Acc & 98.5 & 84.7 & 60.5 & 82.4 & 47.9 & 86.2 & 39.5 & 65.3 \\
%     \midrule
%     \multirow{3}{}{POS-Brown} & CR & 99.8 & 96.1 & 83.0 & 94.0 & 63.2 & 94.0 & 52.2 & - \\
%     & IR & 4.2 & 26.2 & 59.7 & 32.7 & 84.7 & 26.0 & 84.7 & - \\
%     & Acc & 98.2 & 87.4 & 66.4  & 83.6 & 44.5 & 86.2 & 37.8 & 61.0 \\
%     \midrule
%     \multirow{3}{}{POS-COGS} & CR & 100 & 100 & 99.3 & 99.9 & 95.4 & 99.9 & 98.7 & - \\
%     & IR & 0.0 & 1.1 & 10.2 & 2.1 & 89.2 & 84.4 & 89.2 & - \\
%     & Acc & 100 & 99.8 & 97.9 & 99.6 & 83.3 & 87.9 & 86.2 & 85.7 \\
%     \midrule
%     \multirow{3}{}{Syn-WSJ} & CR & {96.9} &84.6 & 61.6 & 66.3 & 38.8 & 66.2 & 20.5 & - \\
%     & IR & 37.9 & 69.6 & 89.9 & 86.5 & 97.0 &  73.1 & 97.0 & - \\
%     & Acc & 75.2& 50.8 & 29.5 & 33.4 & 16.5 & 40.2 & 9.6 & 37.6 \\
%     \midrule
%     \multirow{3}{}{Syn-Brown} & CR & 97.4 & 85.6 & 65.7 & 69.3 & 44.6 & 69.3 & 29.7 & - \\
%     & IR & 42.6 & 70.7 & 88.0 & 85.7 & 96.0 &  73.9 & 96.0 & - \\
%     & Acc & 70.9 & 48.3 & 30.2 & 32.9 & 17.7 & 40.7 & 12.7 & 33.8 \\
%     \bottomrule
%     \end{tabularx}
%     \caption{Predicted test-set accuracy with different methods. \textit{Maxprob} refers to using the maximum predicted probability as discriminator.  \textit{Upper.} and \textit{Lower.} refers to predicted upperbound and lowerbound. \textit{Gold} refers to the accuracy evaluated with gold annotations. 
%     \textit{Maxprob (Oracle)} means that we assume we can set the threshold to make the \textit{Maxprob} method sharing the same \textit{Correct-Recall} score with \textit{Upper.} under \textit{Ours} or the same \textit{Incorrect-Recall} score 
%     with  \textit{Lower.} under \textit{Ours}. This method is mainly reported to make comparison with our discriminators.
%     }
%     \label{tab:discrim:test_acc}
% \end{table*}



% \begin{table*}
% \footnotesize
%     \centering
%     \begin{tabularx}{\linewidth}{XXXXXXXXXX}
%     \toprule
%      &  & \multicolumn{1}{c}{\textit{Maxprob}} & \multicolumn{2}{c}{\textit{Maxprob (Oracle)}} & \multicolumn{3}{c}{Ours} & \textit{AC} & Gold \\
%      \cmidrule(lr){3-3}
%      \cmidrule(lr){4-5}
%      \cmidrule(lr){6-8}
%      % \cmidrule(lr){9-9}
%     Data & Metric & $\gamma$=0.5 & Upper. & Lower. & Upper. & Lower. & Mean & &\\ 
%     \midrule
%     \multirow{4}{*}{MCD1} & CR  & 98.7  & 99.2 & 71.7 & 99.2 & 92.9 & - & - &- \\
%     & IR  & 35.0 & 31.2 & 94.5 & 69.8 & 94.5 & - & -& -\\
%     & Acc & 84.5 & 86.4 & 43.7 & 70.0 & 56.0 & 63.0 & 82.5 & 57.8 \\
%     & MAE & 26.7 & - & - & - & - & \textbf{5.2} & 24.7 & - \\
%     \midrule
%     \multirow{4}{*}{MCD2} & CR  & 96.7 & 83.4 & 48.7 & 83.4 & 71.7 & -& - &-  \\
%     & IR & 27.6  & 58.3 & 92.2 & 77.9 & 92.2 & -& - &- \\
%     & Acc& 78.0 & 51.3 & 17.2 & 36.1 & 22.4 & 29.3 & 74.0 & 22.9 \\
%     & MAE & 55.1 & - & - & - & - & \textbf{6.4} & 51.1 & - \\

%     \midrule
%     \multirow{4}{*}{COGS} & CR & 99.8 & 99.8 & 48.2 & 99.8 & 98.5 & -& -& - \\
%     & IR & 32.0 & 36.6 & 96.9 & 89.4 & 96.9 & -& -& - \\
%     & Acc & 97.1 & 96.7 & 44.3 & 92.1 & 90.2 & 91.2 & 96.6 & 91.4\\
%     & MAE & 5.7 & - & - & - & - & \textbf{0.3} & 5.2 & - \\

%     \midrule
%     \multirow{4}{*}{Top} & CR  & 98.1 & 92.2 & 81.6 & 92.2 & 82.5 & -& - &- \\
%     & IR & 23.7 & 31.6 & 78.9 & 44.7 & 78.9 & - & - &-\\
%     & Acc & 92.2 & 85.8 & 65.2 & 82.3 & 66.0 & 74.2 & 85.9 & 73.0 \\
%     & MAE & 19.2 & - & - & - & - & \textbf{1.2} & 12.9 & - \\
%     \midrule
%     \multirow{4}{*}{AMR} & CR & 96.4& 71.0 & 35.2 & 70.9 & 29.1 & - & -& -\\
%     & IR & 67.2 & 90.9 & 99.1 & 84.1 & 99.1 & -& - & -\\
%     & Acc& 40.6 & 17.9 & 5.8 & 22.6 & 4.5 & 13.6 & 38.0 & 12.2 \\
%     & MAE & 28.4 & - & - & - & - & \textbf{1.4} & 25.8 & - \\
%     \midrule
%     \multirow{4}{*}{POS-WSJ} & CR & 94.4 & 93.0 & 65.3 & 93.0 & 52.4 & - & - & -\\
%     & IR & 33.3 & 37.5 & 84.8 &  26.5 & 84.8 & - & -& -\\
%     & Acc& 84.7 & 82.4 & 47.9 & 86.2 & 39.5 & 62.9 & 77.4 & 65.3 \\
%     & MAE & 19.4 & - & - & - & - & \textbf{2.5} & 12.1 & - \\
%     \midrule
%     \multirow{4}{*}{POS-Brown} & CR & 96.1 & 94.0 & 63.2 & 94.0 & 52.2 & - & - & -\\
%     & IR & 26.2 & 32.7 & 84.7 & 26.0 & 84.7 & -& - & - \\
%     & Acc & 87.4 & 83.6 & 44.5 & 86.2 & 37.8 & 62.0 & 80.5& 61.0 \\
%     & MAE & 26.4 & - & - & - & - & \textbf{1.0} & 19.5 & - \\
%     \midrule
%     \multirow{4}{*}{POS-COGS} & CR& 100 & 99.9 & 95.4 & 99.9 & 98.7 & -& - & - \\
%     & IR & 1.1 & 2.1 & 89.2 & 84.4 & 89.2 & -& - & - \\
%     & Acc & 99.8 & 99.6 & 83.3 & 87.9 & 86.2 & 87.1 & 100 & 85.7 \\
%     & MAE & 14.1 & - & - & - & - & \textbf{1.4} & 14.3 & - \\
%     \midrule
%     \multirow{4}{*}{Syn-WSJ} & CR &84.6& 66.3 & 38.8 & 66.2 & 20.5 & - & - & -\\
%     & IR  & 69.6 & 86.5 & 97.0 &  73.1 & 97.0 & - & - & -\\
%     & Acc & 50.8 & 33.4 & 16.5 & 40.2 & 9.6 & 24.9 & 52.4 & 37.6 \\
%     & MAE & 13.2 & - & - & - & - & \textbf{12.7} & 14.8 & - \\
%     \midrule
%     \multirow{4}{*}{Syn-Brown} & CR & 85.6 & 69.3 & 44.6 & 69.3 & 29.7 & - & - & -\\
%     & IR & 70.7 & 85.7 & 96.0 &  73.9 & 96.0 & - & - & -\\
%     & Acc & 48.3 & 32.9 & 17.7 & 40.7 & 12.7 & 26.7 & 50.8 & 33.8 \\
%     & MAE & 14.5 & - & - & - & - & \textbf{7.1} & 17.0 & - \\
%     \bottomrule
%     \end{tabularx}
%     \caption{Predicted test-set accuracy with different methods. 
%     For each dataset, we report \textit{Correct-Recall} (CR), \textit{Incorrect-Recall} (IR), predicted accuracy (Acc) and MAE scores. 
%     \textit{Maxprob} refers to using the maximum predicted probability as discriminator.  \textit{Upper.} and \textit{Lower.} refers to predicted upperbound and lowerbound. 
%     \textit{AC} refers to average confidence baseline. 
%     \textit{Gold} refers to the accuracy evaluated with gold annotations. 
%     \todo{This table is now a bit large and we still want to include more comparable baseline methods.}
%     % \textit{Maxprob (Oracle)} means that we assume we can set the threshold to make the \textit{Maxprob} method sharing the same \textit{Correct-Recall} score with \textit{Upper.} under \textit{Ours} or the same \textit{Incorrect-Recall} score 
%     % with  \textit{Lower.} under \textit{Ours}. This method is mainly reported to make comparison with our discriminators.
%     }
%     \label{tab:discrim:test_acc}
% \end{table*}


\begin{table*}[!htp]\centering
\footnotesize
\begin{tabularx}{\linewidth}{XXXXXXXXXXX}
\toprule
& \multicolumn{8}{c}{OOD} & \multicolumn{2}{c}{IID} \\
\cmidrule(lr){2-9}
\cmidrule(lr){10-11}
&\multicolumn{2}{c}{MCD1} &\multicolumn{2}{c}{MCD2} &\multicolumn{2}{c}{COGS} &\multicolumn{2}{c}{TOP} &\multicolumn{2}{c}{AMR 2.0} \\\cmidrule{2-11}
&Acc &MAE &Acc &MAE &Acc &MAE &Acc &MAE &Acc &MAE \\\midrule
\multicolumn{11}{c}{Maxprob} \\
\midrule
% $\gamma=$0.25 &95.5 &37.7 &94.0 &71.1 &99.5 &8.1 &99.3 &26.3 &61.9 &47.6 \\
$\gamma=$0.5 &84.5 &71.7 &78.0 &55.1 &97.1 &5.7 &92.2 &19.2 &40.6 &26.3 \\
% $\gamma=$0.75 &71.7 &13.9 &57.0 &34.1 &94.4 &3.0 &72.3 &0.7 &26.1 &11.8 \\
\midrule
\multicolumn{11}{c}{Maxprob (Oracle)} \\
\midrule
Upper. &86.4 &- &51.3 &- &96.7 &- &85.8 &- &17.9 &- \\
Lower. &43.7 &- &17.2 &- &44.3 &- &65.2 &- &5.8 &- \\
Mean &65.1 &7.3 &34.3 &11.4 &70.5 &20.9 &75.5 &2.5 &11.8 &2.5 \\
\midrule
\multicolumn{11}{c}{Previous methods} \\
\midrule
\textit{AC} &82.5 &24.7 &74.0 &51.1 &96.6 &5.2 &85.9 &12.9 &38.0 &23.7 \\
\textit{ATC} &73.0 &15.2 &56.9 &34.0 &100.0 &8.6 &66.0 &7.0 &15.5 &1.2 \\
\midrule
\multicolumn{11}{c}{Ours} \\
\midrule
Upper. &70.0 &- &36.1 &- &92.1 &- &82.3 &- &22.6 &- \\
Lower. &56.0 &- &22.4 &- &90.2 &- &66.0 &- &4.5 &- \\
Mean &63.0 &\textbf{5.2} &29.3 &\textbf{6.4} &91.2 &\textbf{0.3} &74.2 &\textbf{1.2} &13.6 &\textbf{0.8} \\
\midrule

Gold &57.8 &0.0 &22.9 &0.0 &91.4 &0.0 &73.0 &0.0 &14.3 &0.0 \\
\bottomrule
\end{tabularx}
\caption{Predicted test-set accuracy with different methods. 
    For each dataset, we report \textit{Correct-Recall} (CR), \textit{Incorrect-Recall} (IR), predicted accuracy (Acc) and MAE scores. 
    \textit{Maxprob} refers to using the maximum predicted probability as discriminator.  \textit{Upper.} and \textit{Lower.} refers to predicted upperbound and lowerbound. 
    \textit{AC} refers to average confidence baseline. 
    \textit{Gold} refers to the accuracy evaluated with gold annotations. 
}
\label{tab:discrim:sem_acc}
\end{table*}


\begin{table}[!htp]\centering
\footnotesize
\begin{tabularx}{\linewidth}{XXXXXXX}\toprule
& \multicolumn{4}{c}{OOD} & \multicolumn{2}{c}{IID} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-7}
&\multicolumn{2}{c}{POS-Brown} &\multicolumn{2}{c}{POS-COGS} &\multicolumn{2}{c}{POS-WSJ} \\\cmidrule{2-7}
&Acc &MAE &Acc &MAE &Acc &MAE \\
\midrule
\multicolumn{7}{c}{Maxprob} \\\midrule
$\gamma=$0.5 &87.4 &26.4 &99.8 &14.1 &84.7 &19.4 \\\midrule
\multicolumn{7}{c}{Maxprob (Oracle)} \\\midrule
Upper. &83.6 &- &99.6 &- &82.4 &- \\
Lower. &44.5 &- &83.3 &- &47.9 &- \\
Mean &64.0 &3.0 &91.4 &5.7 &65.2 &\textbf{0.1} \\\midrule
\multicolumn{7}{c}{Previous methods} \\\midrule
\textit{AC} &80.5 &19.5 &100.0 &14.3 &77.4 &12.1 \\
\textit{ATC} &68.0 &7.0 &100.0 &14.3 &61.6 &3.7 \\\midrule
\multicolumn{7}{c}{Ours} \\\midrule
Upper. &86.2 &- &87.9 &- &86.2 &- \\
Lower. &37.8 &- &86.2 &- &39.5 &- \\
Mean &62.0 &\textbf{1.0} &87.1 &\textbf{1.4} &62.9 &2.4 \\\midrule
Gold &61.0 &0.0 &85.7 &0.0 &65.3 &0.0 \\
\bottomrule
\end{tabularx}
\caption{Predicted test-set accuracy for POS tagging tasks.}
\label{tab:discrim:pos_acc}
\end{table}

\begin{table}[!htp]\centering
\footnotesize
\begin{tabularx}{\linewidth}{XXXXX}\toprule
&\multicolumn{2}{c}{OOD} &\multicolumn{2}{c}{IID} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
&\multicolumn{2}{c}{Syn-Brown} &\multicolumn{2}{c}{Syn-WSJ} \\\cmidrule{2-5}
&Acc &MAE &Acc &MAE \\\midrule
\multicolumn{5}{c}{Maxprob} \\\midrule
$\gamma=$0.5 &50.8 &13.2 &48.3 &14.5 \\\midrule
\multicolumn{5}{c}{Maxprob (Oracle)} \\\midrule
Upper. &33.4 &- &32.9 &- \\
Lower. &16.5 &- &17.7 &- \\
Mean &24.9 &12.7 &25.3 &8.5 \\\midrule
\multicolumn{5}{c}{Previous methods} \\\midrule
\textit{AC} &52.4 &14.8 &50.8 &17.0 \\
\textit{ATC} &34.0 &\textbf{3.6} &34.7 &\textbf{0.9} \\\midrule
\multicolumn{5}{c}{Ours} \\\midrule
Upper. &40.2 &- &40.7 &- \\
Lower. &9.6 &- &12.7 &- \\
Mean &24.9 &12.7 &26.7 &7.1 \\\midrule
Gold &37.6 &0.0 &33.8 &0.0 \\
\bottomrule
\end{tabularx}
\caption{Predicted test-set accuracy for constituency parsing tasks.}
\label{tab:discrim:syn_acc}
\end{table}

==> tables/discrim_results.tex <==
\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{XXXXXXX}
    \toprule
     & & \multicolumn{5}{c}{GeoQuery} \\
     \midrule
     Model & Train data & Auc & CP & CR & IP & IR \\
    \midrule
    T5 & Random & 70 & 88 & 99 & 88 & 32 \\ 
    T5 & Model & 78 & 86 & 99 & 83 & 21 \\
    \midrule
    & & \multicolumn{5}{c}{MCD1} \\
    \midrule
    T5 & Random & 91 & 73 & 99 & 88 & 50 \\ 
    T5 & Model & 96 & 85 & 98 & 97 & 76 \\
    \midrule
    & & \multicolumn{5}{c}{COGS} \\
    \midrule
    T5 & Model & 93 & 97 & 100 & 99 & 72 \\
    \bottomrule
    \end{tabularx}
    \caption{Results of discriminators. \textit{CP, CR, IP, IR} refer to \textit{Correct Precision}, \textit{Correct-Recall}, \textit{Incorrect-Precision} and \textit{Incorrect-Recall} respectively. 
    % \todo{plan to add results with additional MRs from dev set.} 
    % \todo{update numbers}
    }
    \label{tab:discrim_results}
\end{table}


\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{XXXXXX}
    \toprule
     &  & & & \multicolumn{2}{c}{MCD1} \\
     \cmidrule(lr){5-6}
    Model & Data & ratio & ens. & CR & IR \\
    \midrule
    T5 & M_{2k} & 1:1 & $\times$1 & 98 & 76 \\
    T5 & M_{2k} & 3:1 & $\times$1 & 96 & 84 \\
    T5 & M_{2k} & 9:1 & $\times$1 & 96 & 87 \\
    T5 & M_{2k} & 9:1 & $\times$3 & 91 & 92 \\
    T5 & M_{2k} & 9:1 & $\times$5 & 89 & \textbf{95} \\
    Roberta & M_{2k} & 1:1 & $\times$1 & 96 & 76 \\
    \midrule
    & & & & \multicolumn{2}{c}{MCD2} \\
    \cmidrule(lr){5-6}
     Model & Data & ratio & ens. & CR & IR \\
    \midrule
    T5 & M_{2k} & 1:1 & $\times$1 & 86 & 79 \\
    T5 & M_{2k} &3:1 & $\times$1 & 82 & 80 \\
    T5 & M_{2k} &3:1 & $\times$3 & 78 & 85 \\
    T5 & M_{2k} &3:1 & $\times$5 & 76 & \textbf{89} \\
    \bottomrule
    \end{tabularx}
    \caption{Results of discriminators on CFQ with different settings. \textit{Data} refers to the method we use to prepare our training data. \textit{ratio} refers to the ratio of negatives to positive samples in the training data. \textit{ens.} refers to the number of models used to do ensemble.  }
    % \todo{Sorry that the table is still messy. I am now running more experiments to make fair comparison.} }
    \label{tab:discrim_cfq_results}
\end{table}


\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{XXXXXX}
    \toprule
         & & & &\multicolumn{2}{c}{COGS} \\
         \cmidrule(lr){5-6}
     Model & Data & ratio & ens. & CR & IR \\
    \midrule
    T5 & M_{25k} &1:1 & $\times$1 & 100 & 72 \\
    T5 & M_{25k} &3:1 & $\times$1 & 98 & 78 \\
    T5 & M_{25k} &3:1 & $\times$3 & 98 & 78 \\
    T5 & M_{25k} &3:1 & $\times$5 & 98 & 78 \\
    T5 & M_{0.5k} &3:1 & $\times$1 & 100 & 88 \\
    T5 & M_{0.5k} &3:1 & $\times$3 & 100 & 93 \\
    T5 & M_{0.5k} &3:1 & $\times$5 & 100 & \textbf{94} \\
    \bottomrule
    \end{tabularx}
    \caption{Results of discriminators on COGS with different settings. 
    % \todo{I also tried to ensemble models trained on different data (i.e.\ $M_{25k}$ and $M_{0.5k}$), which yields the best IR (i.e.\ 94\%) on COGS so far}
    }
    \label{tab:discrim_cogs_results}
\end{table}

% \begin{table}
% \footnotesize
%     \centering
%     \begin{tabularx}{\linewidth}{XXX}
%     \toprule
%      \multicolumn{3}{c}{MCD1} \\
%     Upper. & Lower. & Acc \\
%     \midrule
%     61.2 & 53.4 & 57.8 \\
%     \midrule
%     \multicolumn{3}{c}{MCD2} \\
%     Upper. & Lower. & Acc \\
%     \midrule
%     33.5 & 25.5 & 22.9 \\
%     \midrule
%     \multicolumn{3}{c}{COGS} \\
%     Upper. & Lower. & Acc \\
%     \midrule
%      92.1 & 91.6 & 91.4 \\
%     \bottomrule
%     \end{tabularx}
%     \caption{Predicted upperbound and lowerbound accuracy on the test set. 
%     \textit{Upper.} refers to the predicted upperbound. 
%     \textit{Lower.} refers to the predicted lowerbound.
%     \textit{Acc} refers to the accuracy evaluated on the gold test set. 
%     \todo{For most models both the \textit{Correct-recall} and \textit{Incorrect-recall} is high so the predicted accuracy is already very close to realistic accuracy.}
%     }
%     \label{tab:discrim_pred_acc}
% \end{table}




==> tables/ls_results.tex <==
\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{lXXXX}
    \toprule
     & GeoQuery & MCD1 & MCD2 & COGS\\
     % \cmidrule{}
    \midrule
    T5 (beam size=20) & 75 & 99 & 70 & 83 \\ 
    \bottomrule
    \end{tabularx}
    \caption{Results of Local structure prediction.
    }
    \label{tab:ls_results}
\end{table}

\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{lXX}
    \toprule
     Model & Setting& MCD1 \\
     % \cmidrule{}
    \midrule
    \multirow{4}{*}{T5} & baseline & 58 \\ 
    & M1 & 50 \\
    & M2 & 58 \\
    & M3 & \textbf{77} \\
    \bottomrule
    \end{tabularx}
    \caption{Exact match accuracy of T5 with different ways to exploit local structures.
    }
    \label{tab:ls_exploit_results}
\end{table}

==> tables/refine_results.tex <==
\begin{table}
\footnotesize
    \centering
    \begin{tabularx}{\linewidth}{lXXX}
    \toprule
     & COGS & CFQ & GeoQuery \\
     % \cmidrule{}
    \midrule
    T5 & - & 62 & 81 \\ 
    \bottomrule
    \end{tabularx}
    \caption{Exact match accuracy of refine models.
    }
    \label{tab:refine_results}
\end{table}
